On canonical bases and induction of $W$-graphs

A canonical basis in the sense of Lusztig is a basis of a free module over a ring of Laurent polynomials that is invariant under a certain semilinear involution and is obtained from a fixed "standard basis" through a triangular base change matrix with polynomial entries whose constant terms equal the identity matrix. Among the better known examples of canonical bases are the Kazhdan-Lusztig basis of Iwahori-Hecke algebras, Lusztig's canonical basis of quantum groups and the Howlett-Yin basis of induced $W$-graph modules. This paper has two major theoretical goals: First to show that having bases is superfluous in the sense that canonicalisation can be generalized to non-free modules. This construction is functorial in the appropriate sense. The second goal is to show that Howlett-Yin induction of $W$-graphs is well-behaved a functor between module categories of $W$-graph-algebras that satisfies various properties one hopes for when a functor is called "induction", for example transitivity and a Mackey theorem.

==> _preamble/language_de.tex <==
%%% Language preamble for german

% Language itself
\usepackage[ngerman]{babel}
% Font encoding to represent umlauts correct in PDFs documents instead of combining them from other
% characters like "u instead of ü
\usepackage[T1]{fontenc}
% Encoding of the source code.
\usepackage[utf8]{inputenc}


% Language specific strings
%   Names of theorem environments
\newcommand{\captionstringtheorem}{Satz}
\newcommand{\captionstringlemma}{Lemma}
\newcommand{\captionstringcorollary}{Korollar}
\newcommand{\captionstringlemmadef}{Lemma und Definition}
\newcommand{\captionstringtheoremdef}{Satz und Definition}
\newcommand{\captionstringdefinition}{Definition}
\newcommand{\captionstringproposition}{Proposition}
\newcommand{\captionstringexample}{Beispiel}
\newcommand{\captionstringconjecture}{Vermutung}
\newcommand{\captionstringconvention}{Vereinbaring}
\newcommand{\captionstringremark}{Bemerkung}


